GADT meet Subtyping

While generalized abstract datatypes (GADT) are now considered well-understood, adding them to a language with a notion of subtyping comes with a few surprises. What does it mean for a GADT parameter to be covariant? The answer turns out to be quite subtle. It involves fine-grained properties of the subtyping relation that raise interesting design questions. We allow variance annotations in GADT definitions, study their soundness, and present a sound and complete algorithm to check them. Our work may be applied to real-world ML-like languages with explicit subtyping such as OCaml, or to languages with general subtyping constraints.

==> rrconf.tex <==
\usepackage{a4}
\usepackage{RR}

\RRNo{8114}
\RRdate{October 2012}

\RRauthor{% les auteurs
Gabriel Scherer
\and
Didier R\'emy
}
%% Ceci apparait sur chaque page paire.
\authorhead{Scherer \& R\'emy}
%% titre francais long
\RRtitle{GADT avec sous-typage}
%% English title
\RRetitle{GADT meet subtyping}
%\titlehead{Example of RR.sty}
%%
\RRnote{Part of this work has been done at IRILL}
%%
\RRresume{
  Les types alg\'ebriques g\'en\'eralis\'es (\textit{Generalized Algebraic
    Datatypes}, \GADTs) sont maintenant bien compris, mais leur ajout
  \`a un langage \'equip\'e de sous-typage nous r\'eservait quelques
  surprises. Qu'est-ce qu'\^etre covariant pour un param\`etre de \GADT?
%
  La r\'eponse s'av\`ere difficile. Elle met en jeu des propri\'et\'es
  fines de la relation de sous-typage qui soul\`event d'int\'eressantes
  probl\'ematiques de conception de langage.
%
  Nous permettons des annotations de variance dans les d\'efinitions de
  \GADTs, \'etudions leur correction, et pr\'esentons un algorithme
  correct et complet pour les v\'erifier. Notre travail peut s'appliquer
  \`a un langage complet inspir\'e de ML et avec sous-typage explicite,
  tel que OCaml, ou m\^eme \`a des langages avec des contraintes g\'en\'erales
  de sous-typage.
}
\RRabstract{
  While generalized abstract datatypes (\GADT) are now considered
  well-understood, adding them to a language with a notion of
  subtyping comes with a few surprises. What does it mean for a \GADT
  parameter to be covariant?
%
  The answer turns out to be quite subtle. It involves fine-grained
  properties of the subtyping relation that raise interesting design
  questions.
%
  We allow variance annotations in \GADT definitions, study their
  soundness, and present a sound and complete algorithm to check them.
  Our work may be applied to real-world ML-like languages with
  explicit subtyping such as OCaml, or to languages with general
  subtyping constraints.
}
%%
\RRmotcle{sous-typage, types de donn\'ees, variance}
\RRkeyword{subtyping, datatypes, variance}
%%
\RRprojet{Gallium}
%%
%% \URLorraine % pour ceux qui sont \`a l'est
%% \URRennes  % pour ceux qui sont \`a l'ouest
%% \URRhoneAlpes % pour ceux qui sont dans les montagnes
%% \URRocq % pour ceux qui sont au centre de la France
%% \URFuturs % pour ceux qui sont dans le virtuel
%% \URSophia % pour ceux qui sont au Sud.
%%
%% \RCBordeaux % centre de recherche Bordeaux - Sud Ouest
%% \RCLille % centre de recherche Lille Nord Europe
\RCParis % Paris Rocquencourt
%% \RCSaclay % Saclay \^Ile de France
%% \RCGrenoble % Grenoble - Rh\^one-Alpes
%% \RCNancy % Nancy - Grand Est
%% \RCRennes % Rennes - Bretagne Atlantique
%% \RCSophia % Sophia Antipolis M\'editerran\'ee

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "RR-8114"
%%% End: 

